HERA Phase I Limits on the Cosmic 21-cm Signal: Constraints on Astrophysics and Cosmology During the Epoch of Reionization

Recently, the Hydrogen Epoch of Reionization Array (HERA) collaboration has produced the experiment's first upper limits on the power spectrum of 21-cm fluctuations at z~8 and 10. Here, we use several independent theoretical models to infer constraints on the intergalactic medium (IGM) and galaxies during the epoch of reionization (EoR) from these limits. We find that the IGM must have been heated above the adiabatic cooling threshold by z~8, independent of uncertainties about the IGM ionization state and the nature of the radio background. Combining HERA limits with galaxy and EoR observations constrains the spin temperature of the z~8 neutral IGM to 27 K < T_S < 630 K (2.3 K < T_S < 640 K) at 68% (95%) confidence. They therefore also place a lower bound on X-ray heating, a previously unconstrained aspects of early galaxies. For example, if the CMB dominates the z~8 radio background, the new HERA limits imply that the first galaxies produced X-rays more efficiently than local ones (with soft band X-ray luminosities per star formation rate constrained to L_X/SFR = { 10^40.2, 10^41.9 } erg/s/(M_sun/yr) at 68% confidence), consistent with expectations of X-ray binaries in low-metallicity environments. The z~10 limits require even earlier heating if dark-matter interactions (e.g., through millicharges) cool down the hydrogen gas. Using a model in which an extra radio background is produced by galaxies, we rule out (at 95% confidence) the combination of high radio and low X-ray luminosities of L_{r,\nu}/SFR > 3.9 x 10^24 W/Hz/(M_sun/yr) and L_X/SFR<10^40 erg/s/(M_sun/yr). The new HERA upper limits neither support nor disfavor a cosmological interpretation of the recent EDGES detection. The analysis framework described here provides a foundation for the interpretation of future HERA results.

==> H1C_Theory_arXiv update/defns.tex <==
\newcommand{\note}[1]{{\color{red} #1}}
\newcommand{\tdyn}{t_{\rm dyn}}
\newcommand{\Mhalo}{M_{\rm h}}
\newcommand{\aveMhalo}{\bar{M}_{\rm h}}
\newcommand{\nlea}{\bar{n}_{\rm LAE}}
\newcommand{\zpeak}{z_{\rm peak}}
\newcommand{\taure}{\tau_{\rm reion}}
\newcommand{\tauHII}{\tau_{\rm HII}}
\newcommand{\Dss}{\Delta_{\rm ss}}
\newcommand{\Dmod}{\Delta_{\rm mod}}
\newcommand{\Dextr}{\Delta_{\rm extr}}
\newcommand{\GammaHII}{\Gamma_{\rm HII}}
\newcommand{\aveGammaHII}{\langle \Gamma_{12} \rangle_{\rm HII}}
\newcommand{\avenfHII}{\langle x_{\rm HI} \rangle_{\rm HII}}
\newcommand{\fesc}{f_{\rm esc}}
\newcommand{\QHII}{Q_{\rm HII}}
\newcommand{\qnamesevenone}{ULAS J1120+0641}
\newcommand{\sense}{\textsc{\small 21cmsense}}
\newcommand{\dexm}{\textsc{\small DexM}}
\newcommand{\enzo}{\textsc{\small ENZO}}
\newcommand{\Zsun}{Z_\odot}
\newcommand{\uunit}{{\bf \hat{u}}}
\newcommand{\cmfast}{{\tt 21cmFAST}}
\newcommand{\cmmc}{{\tt 21cmMC}}
\newcommand{\muKK}{\mu {\rm K^2}}
\newcommand{\PkSZ}{[\Delta^{\rm patchy}_{l3000}]^2}
\newcommand{\POV}{[\Delta^{\rm OV}_{l3000}]^2}
\newcommand{\Ptot}{[\Delta_{l3000}]^2}
\newcommand{\reionparams}{\{\zeta, T_{\rm vir}, R_{\rm mfp}\}}
\newcommand{\delz}{\Delta z_{\rm re}}
\newcommand{\zre}{z_{\rm re}}
\newcommand{\HI}{\ion{H}{1}}
\newcommand{\HII}{\ion{H}{2}}
\newcommand{\MgII}{\ion{Mg}{2}}
\newcommand{\OVI}{\ion{O}{6}}
\newcommand{\ef}{x_{e^-}}
\newcommand{\frec}{f_{\rm rec}}
\newcommand{\Ndot}{\dot{N}_{\rm X}}
\newcommand{\Omb}{\Omega_{\rm b}}
\newcommand{\xz}{({\bf x}, z)}
\newcommand{\xzp}{({\bf x}, z')}
\newcommand{\Ts}{T_{\rm S}}
\newcommand{\Tk}{T_{\rm K}}
\newcommand{\aveTs}{\overline{T}_{\rm S}}
\newcommand{\aveTk}{\overline{T}_{\rm K}}
\newcommand{\denps}{\Delta^2_{\delta \delta}({\bf k}, z)}
\newcommand{\chisq}{\chi^2}
\newcommand{\htwo}{\mathrm{H}_2}
\newcommand{\hone}{\mathrm{H}\textsc{i}}
\newcommand{\hii}{\mathrm{H}\textsc{ii}}
\newcommand{\nf}{\hone}
\newcommand{\Rom}[1]{\uppercase\expandafter{\romannumeral #1}}
\newcommand{\rom}[1]{\lowercase\expandafter{\romannumeral #1}}
\newcommand{\Mvir}{M_{\rm vir}}
\newcommand{\avenf}{\overline{x}_{\hone}}
\newcommand{\nfIGM}{x_{\hone}^{\rm IGM}}
\newcommand{\strom}{HII region}
\newcommand{\lya}{Ly$\alpha$}
\newcommand{\lyb}{Ly$\beta$}
\newcommand{\taudamp}{\tau_{D}}
\newcommand{\taures}{\tau_{R}}
\newcommand{\lobs}{\lambda_{\rm obs}}
\newcommand{\tauobs}{\tau_{\rm obs}}
\newcommand{\tausim}{\tau_{\rm sim}}
\newcommand{\zsource}{z_{\rm s}}
\newcommand{\lcdm}{$\Lambda$CDM}
\newcommand{\fion}{f_{\rm ion}}
\newcommand{\hs}{\hspace{1mm}}
\newcommand{\qnamesfourtwo}{SDSS J1148+5251}
\newcommand{\qnamestwoeight}{SDSS J1030+0524}
\newcommand{\qnamestwotwo}{SDSS J1623+3112}
\newcommand{\qnamestwo}{SDSS J1048+4637}
\newcommand{\qnamefourtwo}{J1148+5251}
\newcommand{\qnametwoeight}{J1030+0524}
\newcommand{\qnametwotwo}{J1623+3112}
\newcommand{\qnametwo}{J1048+4637}
\newcommand{\taub}{\tau_{\rm lim(Ly\beta)}}
\newcommand{\taua}{\tau_{\rm lim(Ly\alpha)}}
\newcommand{\tautot}{\tau_{\rm Ly\alpha}} 
\newcommand{\fobs}{f_\nu^{obs}}
\newcommand{\fcon}{f_\nu^{con}}
\newcommand{\fgamma}{f_\Gamma}
\newcommand{\deltakvec}{\delta({\bf k})}
\newcommand{\deltaxvec}{\delta({\bf x})}
\newcommand{\sigsq}{\sigma^2(M)}
\newcommand{\sig}{\sigma(M)}
\newcommand{\delc}{\delta_c(M,z)}
\newcommand{\Msun}{M_\odot}
\newcommand{\Tvir}{T_{\rm vir}}
\newcommand{\Tvirmin}{T_{\rm vir}^{\rm min}}
\newcommand{\fcoll}{f_{\rm coll}(z, >M_{\rm halo})}
\newcommand{\fcollEPS}{f_{\rm coll}({\bf x}, z, R)}
%\newcommand{\fcoll}{f_{\rm gas}}
\newcommand{\deltanlxvec}{\delta_{\rm nl}({\bf x_1}, z)}
\newcommand{\Tcmb}{T_\gamma}
\newcommand{\avedelT}{\bar{\delta T_b}}
\newcommand{\delT}{\delta T_b}
\newcommand{\deldelT}{\delta_{\rm 21}}
\newcommand{\delNL}{\delta_{\rm nl}}
\newcommand{\Mmin}{M_{\rm min}}
\newcommand{\Mwdm}{m_{\rm wdm}}
\newcommand{\mfp}{R_{\rm mfp}}
\newcommand{\zbegin}{z_{\rm begin}}
\newcommand{\zend}{z_{\rm end}}
\newcommand{\Tgamma}{T_{\gamma, \rm res}}
\newcommand{\avexi}{\bar{\xi}_{12}}
\newcommand{\zon}{z_{\rm on}}
\newcommand{\lmfp}{\lambda_{\rm mfp}}
\newcommand{\lXmfp}{\lambda^{\rm mfp}_{\rm X}}
\newcommand{\toteff}{\epsilon_{\rm fid}}
\newcommand{\Msum}{\mathcal{M}({\bf x}, z)}
\newcommand{\flux}{f({\bf x}, z)}
\newcommand{\Jcrit}{J^{\rm crit}_{21}(M, z)}
\newcommand{\kmps}{\rm km~s^{-1}}
\newcommand{\taueff}{\tau_{\rm eff}^{\rm GP}}
\newcommand\lsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
        \raise1pt\hbox{$<$}}}
\newcommand\gsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
        \raise1pt\hbox{$>$}}}
\def\myputfigure#1#2#3#4#5%
{\vskip#5pt\makebox[0pt]{\hskip#2in
\includegraphics[width=#3\textwidth]{#1}}\vskip#4pt\hfill}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newcommand{\myurl}{\texttt}
\newcommand{\mytilde}{\texttildelow}
%\newcommand\ion[2]{#1$\;${\scshape{#2}}}%                       % ion, i.e., CII = \ion{C}{ii}

%Journal names
%\newcommand{\apj}{ApJ}
%\newcommand{\apjl}{ApJ}
%\newcommand{\apjs}{ApJS}
%\newcommand{\aap}{A\&A}
%\newcommand{\aj}{AJ}
%\newcommand{\mnras}{MNRAS}
%\newcommand{\pasj}{PASJ}
%\newcommand{\physrep}{Physics Reports}
%\newcommand{\prd}{PRD}
%\newcommand{\prl}{PRL}
%\newcommand{\nat}{Nature}
%\newcommand{\araa}{ARAA}
%\newcommand{\jcap}{JCAP}
%\newcommand{\pasa}{PASA}
%\newcommand{\nar}{NAR}

